Threshold-Independent Fair Matching through Score Calibration

Entity Matching (EM) is a critical task in numerous fields, such as healthcare, finance, and public administration, as it identifies records that refer to the same entity within or across different databases. EM faces considerable challenges, particularly with false positives and negatives. These are typically addressed by generating matching scores and apply thresholds to balance false positives and negatives in various contexts. However, adjusting these thresholds can affect the fairness of the outcomes, a critical factor that remains largely overlooked in current fair EM research. The existing body of research on fair EM tends to concentrate on static thresholds, neglecting their critical impact on fairness. To address this, we introduce a new approach in EM using recent metrics for evaluating biases in score based binary classification, particularly through the lens of distributional parity. This approach enables the application of various bias metrics like equalized odds, equal opportunity, and demographic parity without depending on threshold settings. Our experiments with leading matching methods reveal potential biases, and by applying a calibration technique for EM scores using Wasserstein barycenters, we not only mitigate these biases but also preserve accuracy across real world datasets. This paper contributes to the field of fairness in data cleaning, especially within EM, which is a central task in data cleaning, by promoting a method for generating matching scores that reduce biases across different thresholds.

==> extra-exp.tex <==

    




\begin{table*}[h]\centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{llllll}\\
    \toprule
     \multirow{2}{*}{\rotatebox[origin=c]{90}{\small Dataset}} & \multirow{2}{*}{Method}  & \multicolumn{3}{c}{Distributional Parity} & \multicolumn{1}{c}{\multirow{2}{*}} \\
    \cmidrule(lr){3-5} 
     & & \DP & \EO & \EOD &\\
    \midrule




    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \amzgog~}}
    & \ditto & 2.37 \stockdown{4.8} & 5.83 \, \stockdown{6.57} & 6.46  \, \stockdown{8.24} \\
    & \hiergat & 6.64 \stockdown{4.45} & 11.60 \stockdown{5.73} & 12.20 \stockdown{9.37} \\
    & \dmatcher & 3.46 \stockdown{5.06} & 10.34 \stockdown{1.39} & 11.19 \stockdown{4.03} \\
    & \hmatcher & 5.03 \stockdown{3.61} & 8.03 \, 
 \stockdown{9.56} & 8.35 \,  \stockdown{12.48} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \walamz~}}
    & \ditto & 2.51 \stockdown{0.84} & 9.72 \, \stockdown{2.97} & 9.76  \, \stockdown{2.53} \\
    & \hiergat & 2.59 \stocknochange & 14.64  \stocknochange & 13.45  \stocknochange \\
    & \dmatcher & 3.44 \stockdown{0.13} & 16.10 \stockdown{15.7} & 16.73 \stockdown{14.49} \\
    & \hmatcher & 2.15 \stocknochange & 11.99 \stocknochange & 12.08 \stocknochange \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPGogS~}}
    & \ditto & 4.00 \stockdown{0.18} & 1.99 \stockdown{0.2} & 2.62 \stocknochange \\
    & \hiergat & 3.41 \stockdown{1.14} & 1.17 \stockdown{2.29} & 1.53 \stockdown{1.44} \\
    & \dmatcher & 4.71 \stockdown{1.0} & 8.32 \stockdown{0.29} & 6.96 \stockdown{1.36} \\
    & \hmatcher & 3.36 \stockdown{1.4} & 3.28 \stockdown{0.36} & 3.51 \stockdown{0.15} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPACM~}}
    & \ditto & 1.06 \stocknochange & 0.55 \stocknochange & 0.52 \stocknochange \\
    & \hiergat & 0.82 \stockdown{0.11} & 0.79 \stockdown{0.45} & 0.64 \stockdown{0.3} \\
    & \dmatcher & 0.64 \stocknochange & 0.51 \stocknochange & 0.54 \stocknochange \\
    & \hmatcher & 0.81 \stocknochange & 1.05 \stocknochange & 1.19 \stocknochange \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \itunamz~}}
    & \ditto & 11.52 \stocknochange & 20.11 \stockdown{3.07} & 22.67 \stockdown{0.58} \\
    & \hiergat & 13.14 \stockdown{6.29} & 24.39 \stockdown{15.68} & 27.14 \stockdown{19.0} \\
    & \dmatcher & 3.80  \, \stockdown{6.6} & 7.07  \, \stockdown{1.73} & 8.18  \, \stockdown{4.88} \\
    & \hmatcher & 1.12  \, \stocknochange& 4.22 \, \stocknochange & 3.97 \, \stocknochange \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \FodorZag~}}
    & \ditto & 2.30 \stocknochange & 6.92 \, \stocknochange & 6.94 \, \stocknochange \\
    & \hiergat & 2.60 \stocknochange & 4.12  \, \stocknochange & 4.12 \, \stocknochange \\
    & \dmatcher & 2.77 \stockdown{1.2} & 12.77 \stockdown{6.46} & 13.51 \stockdown{5.94} \\
    & \hmatcher & 2.45 \stockdown{0.75} & 2.79 \,  \stockdown{4.99} & 6.18  \, \stockdown{2.97} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \Beer~}}
    & \ditto & 18.82 \stockdown{21.37} & 2.12   \, \stocknochange & 17.44 \stockdown{13.75} \\
    & \hiergat & 33.40 \stockdown{2.69} & 34.38 \stockdown{10.02} & 47.05 \stockdown{12.62} \\
    & \dmatcher & 7.59  \, \stockdown{19.08} & 6.65  \, \stockdown{17.33} & 10.95 \stockdown{27.87} \\
    & \hmatcher & 13.30 \stockdown{0.25} & 5.18    \, \stocknochange & 10.95  \stocknochange \\
    

    \bottomrule
    \end{tabular}
    %}
    \caption{after calibration, each column is minimized separately}
        \vspace{-3mm}
        \label{tab:bias-after21}
    \end{table*}


\begin{table*}[h]\centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{lllllllllllllll}\\
    \toprule
     \multirow{2}{*}{\rotatebox[origin=c]{90}{\small Dataset}} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Distributional Parity} & \multicolumn{1}{c}{\multirow{2}{*}{\rotatebox[origin=c]{0}{\centering \AUC}}} & \multicolumn{1}{c}{\multirow{2}{*}{\rotatebox[origin=c]{0}{\centering \small $\Delta \AUC$}}} & \multicolumn{4}{c}{$\tau=0.5$} & \multicolumn{4}{c}{$\tau=0.9$} \\
    \cmidrule(lr){3-5} \cmidrule(lr){8-11} \cmidrule(lr){12-15}
     & & \DP & \EO & \EOD & & & \DP & \EO & \EOD & F1 & \DP & \EO & \EOD & F1 \\
    \midrule

     




    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \amzgog~}}
    & \ditto & \formatNumber{0.0716837} & \formatNumber{0.1470739} & \formatNumber{0.1240158} & \formatNumber{0.9595086} & \formatNumber{0.0226349} & \formatNumber{0.0706690} & \formatNumber{0.0915573} & \formatNumber{0.0720721} & \formatNumber{0.6503667} & \formatNumber{0.0228267} & \formatNumber{0.1049988} & \formatNumber{0.1013514} & \formatNumber{0.2978723} \\
    & \hiergat & \formatNumber{0.1109689} & \formatNumber{0.2157499} & \formatNumber{0.1732545} & \formatNumber{0.9675409} & \formatNumber{0.0040982} & \formatNumber{0.1110453} & \formatNumber{0.2159766} & \formatNumber{0.1734234} & \formatNumber{0.7306889} & \formatNumber{0.0814606} & \formatNumber{0.2190462} & \formatNumber{0.1959459} & \formatNumber{0.6828087} \\
    & \dmatcher & \formatNumber{0.0852730} & \formatNumber{0.1522372} & \formatNumber{0.1173716} & \formatNumber{0.8498773} & \formatNumber{0.0562260} & \formatNumber{0.0973242} & \formatNumber{0.1719680} & \formatNumber{0.1306306} & \formatNumber{0.6517857} & \formatNumber{0.0730956} & \formatNumber{0.2083929} & \formatNumber{0.1846847} & \formatNumber{0.6071429} \\
    & \hmatcher & \formatNumber{0.0864451} & \formatNumber{0.2082518} & \formatNumber{0.1758266} & \formatNumber{0.9422693} & \formatNumber{0.0060525} & \formatNumber{0.1026011} & \formatNumber{0.3336567} & \formatNumber{0.2995495} & \formatNumber{0.6919831} & \formatNumber{0.0527421} & \formatNumber{0.1073606} & \formatNumber{0.0945946} & \formatNumber{0.5593220} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \walamz~}}
    & \ditto & \formatNumber{0.0334759} & \formatNumber{0.1228968} & \formatNumber{0.1268551} & \formatNumber{0.9615768} & \formatNumber{0.0124636} & \formatNumber{0.0337153} & \formatNumber{0.1427736} & \formatNumber{0.1493506} & \formatNumber{0.8042895} & \formatNumber{0.0292306} & \formatNumber{0.0934748} & \formatNumber{0.0999001} & \formatNumber{0.7966102} \\
    & \hiergat & \formatNumber{0.0258767} & \formatNumber{0.1345393} & \formatNumber{0.1463761} & \formatNumber{0.9600204} & \formatNumber{0.0306233} & \formatNumber{0.0259996} & \formatNumber{0.1556869} & \formatNumber{0.1688312} & \formatNumber{0.7816092} & \formatNumber{0.0288772} & \formatNumber{0.1240960} & \formatNumber{0.1303696} & \formatNumber{0.7771084} \\
    & \dmatcher & \formatNumber{0.0357414} & \formatNumber{0.3122199} & \formatNumber{0.3179715} & \formatNumber{0.8334962} & \formatNumber{0.0585612} & \formatNumber{0.0364163} & \formatNumber{0.3494270} & \formatNumber{0.3591409} & \formatNumber{0.6820809} & \formatNumber{0.0416330} & \formatNumber{0.3101356} & \formatNumber{0.3096903} & \formatNumber{0.6964856} \\
    & \hmatcher & \formatNumber{0.0214808} & \formatNumber{0.1207576} & \formatNumber{0.1198746} & \formatNumber{0.9406378} & \formatNumber{0.0520903} & \formatNumber{0.0229369} & \formatNumber{0.1294780} & \formatNumber{0.1288711} & \formatNumber{0.7896104} & \formatNumber{0.0317548} & \formatNumber{0.0435302} & \formatNumber{0.0369630} & \formatNumber{0.7088608} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPGogS~}}
    & \ditto & \formatNumber{0.0417173} & \formatNumber{0.0261775} & \formatNumber{0.0219021} & \formatNumber{0.9943376} & \formatNumber{0.0043953} & \formatNumber{0.0428128} & \formatNumber{0.0042198} & \formatNumber{0.0079545} & \formatNumber{0.9326568} & \formatNumber{0.0510580} & \formatNumber{0.0560378} & \formatNumber{0.0661616} & \formatNumber{0.9228585} \\
    & \hiergat & \formatNumber{0.0454864} & \formatNumber{0.0297138} & \formatNumber{0.0345875} & \formatNumber{0.9968014} & \formatNumber{0.0034296} & \formatNumber{0.0465956} & \formatNumber{0.0235483} & \formatNumber{0.0353535} & \formatNumber{0.9375294} & \formatNumber{0.0402851} & \formatNumber{0.0153542} & \formatNumber{0.0108586} & \formatNumber{0.8897959} \\
    & \dmatcher & \formatNumber{0.0571128} & \formatNumber{0.0831680} & \formatNumber{0.0860708} & \formatNumber{0.9858279} & \formatNumber{0.0426489} & \formatNumber{0.0650295} & \formatNumber{0.0968939} & \formatNumber{0.0991162} & \formatNumber{0.9515377} & \formatNumber{0.0649309} & \formatNumber{0.1096060} & \formatNumber{0.1117424} & \formatNumber{0.9391471} \\
    & \hmatcher & \formatNumber{0.0475617} & \formatNumber{0.0365997} & \formatNumber{0.0364048} & \formatNumber{0.9958992} & \formatNumber{0.0063953} & \formatNumber{0.0595499} & \formatNumber{0.0548650} & \formatNumber{0.0561869} & \formatNumber{0.9276404} & \formatNumber{0.0526075} & \formatNumber{0.0476417} & \formatNumber{0.0494949} & \formatNumber{0.9031936} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPACM~}}
    & \ditto & \formatNumber{0.0106176} & \formatNumber{0.0051771} & \formatNumber{0.0054879} & \formatNumber{0.9987845} & \formatNumber{0.0008359} & \formatNumber{0.0103183} & \formatNumber{0.0038916} & \formatNumber{0.0060866} & \formatNumber{0.9688889} & \formatNumber{0.0125531} & \formatNumber{0.0129752} & \formatNumber{0.0117131} & \formatNumber{0.9707207} \\
    & \hiergat & \formatNumber{0.0093630} & \formatNumber{0.0093831} & \formatNumber{0.0123838} & \formatNumber{0.9999090} & \formatNumber{0.0003096} & \formatNumber{0.0088361} & \formatNumber{0.0070257} & \formatNumber{0.0102622} & \formatNumber{0.9855072} & \formatNumber{0.0088438} & \formatNumber{0.0130268} & \formatNumber{0.0177996} & \formatNumber{0.9909707} \\
    & \dmatcher & \formatNumber{0.0063796} & \formatNumber{0.0054396} & \formatNumber{0.0051026} & \formatNumber{0.9993873} & \formatNumber{0.0018270} & \formatNumber{0.0068598} & \formatNumber{0.0003691} & \formatNumber{0.0048126} & \formatNumber{0.9854423} & \formatNumber{0.0043971} & \formatNumber{0.0114964} & \formatNumber{0.0067235} & \formatNumber{0.9806157} \\
    & \hmatcher & \formatNumber{0.0081192} & \formatNumber{0.0119347} & \formatNumber{0.0105233} & \formatNumber{0.9995538} & \formatNumber{0.0005278} & \formatNumber{0.0093301} & \formatNumber{0.0047909} & \formatNumber{0.0054496} & \formatNumber{0.9844098} & \formatNumber{0.0110709} & \formatNumber{0.0196499} & \formatNumber{0.0226123} & \formatNumber{0.9830508} \\





    
    \bottomrule
    \end{tabular}
    %}
    \caption{Comparison of matching methods \underline{before} score calibration\mostafa{Didnt you also try \magellan? or other methods? I comment later that we can write 8 page paper. If we do that it might be a good idea to include at least one more method?}}
        \vspace{-3mm}
        \label{tab:bias}
    \end{table*}

\begin{table*}[h]\centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{llllll}\\
    \toprule
     \multirow{2}{*}{\rotatebox[origin=c]{90}{\small Dataset}} & \multirow{2}{*}{Method}  & \multicolumn{3}{c}{Distributional Parity} & \multicolumn{1}{c}{\multirow{2}{*}} \\
    \cmidrule(lr){3-5} 
     & & \DP & \EO & \EOD &\\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \amzgog~}}
    & \ditto & 7.17 & 12.40 & 14.71 \\
    & \hiergat & 11.10 & 17.33 & 21.57 \\
    & \dmatcher & 8.53 & 11.74 & 15.22 \\
    & \hmatcher & 8.64 & 17.58 & 20.83 \\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \walamz~}}
    & \ditto & 3.35 & 12.69 & 12.29 \\
    & \hiergat & 2.59 & 14.64 & 13.45 \\
    & \dmatcher & 3.57 & 31.80 & 31.22 \\
    & \hmatcher & 2.15 & 11.99 & 12.08 \\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPGogS~}}
    & \ditto & 4.17 & 2.19 & 2.62 \\
    & \hiergat & 4.55 & 3.46 & 2.97 \\
    & \dmatcher & 5.71 & 8.61 & 8.32 \\
    & \hmatcher & 4.76 & 3.64 & 3.66 \\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPACM~}}
    & \ditto & 1.06 & 0.55 & 0.52 \\
    & \hiergat & 0.94 & 1.24 & 0.94 \\
    & \dmatcher & 0.64 & 0.51 & 0.54 \\
    & \hmatcher & 0.81 & 1.05 & 1.19 \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \itunamz~}}
    & \ditto & 11.52 & 23.18 & 23.25 \\
    & \hiergat & 19.43 & 40.07 & 46.13 \\
    & \dmatcher & 10.40 & 8.81 & 13.06 \\
    & \hmatcher & 1.12 & 4.22 & 3.97 \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \FodorZag~}}
    & \ditto & 2.30 & 6.92 & 6.94 \\
    & \hiergat & 2.60 & 4.12 & 4.12 \\
    & \dmatcher & 3.97 & 19.24 & 19.45 \\
    & \hmatcher & 3.19 & 7.79 & 9.14 \\
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \Beer~}}
    & \ditto & 40.18 & 2.12 & 31.20 \\
    & \hiergat & 36.09 & 44.40 & 59.68 \\
    & \dmatcher & 26.67 & 23.98 & 38.81 \\
    & \hmatcher & 13.55 & 5.18 & 10.95 \\
    \bottomrule
    \end{tabular}
    %}
    \caption{before calibration}
        \vspace{-3mm}
        \label{tab:bias-after21}
\end{table*}




\begin{table*}[h]\centering
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{llllllllllllllll}\\
    \toprule
     \multirow{2}{*}{\rotatebox[origin=c]{90}{\small Dataset}} & \multirow{2}{*}{Method}  & \multicolumn{3}{c}{Distributional Parity} & \multicolumn{1}{c}{\multirow{2}{*}{\rotatebox[origin=c]{0}{\centering \AUC}}} & \multicolumn{1}{c}{\multirow{2}{*}{\rotatebox[origin=c]{0}{\centering \small $\Delta \AUC$}}} & \multicolumn{4}{c}{$\tau=0.5$} & \multicolumn{4}{c}{$\tau=0.9$} & \multicolumn{1}{c}{\multirow{2}{*}{\rotatebox[origin=c]{0}{\centering \normalsize{$\lambda$}}}}\\
    \cmidrule(lr){3-5} \cmidrule(lr){8-11} \cmidrule(lr){12-15}
     & & \DP & \EO & \EOD & & & \DP & \EO & \EOD & F1 & \DP & \EO & \EOD & F1 \\
    \midrule
    
% \green{$\downarrow$ \formatNumber[round-precision=3]{0.0189946}} & 


    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \amzgog~}}
    & \ditto & \formatNumber[round-precision=4]{0.0526891} & \formatNumber[round-precision=4]{0.0593559} & \formatNumber[round-precision=4]{0.0646262} & \formatNumber[round-precision=4]{0.9584708} & \formatNumber[round-precision=4]{0.0223720} & \formatNumber[round-precision=4]{0.0579399} & \formatNumber[round-precision=4]{0.0315315} & \formatNumber[round-precision=4]{0.0425384} & \formatNumber[round-precision=4]{0.6262626} & \formatNumber[round-precision=4]{0.0214247} & \formatNumber[round-precision=4]{0.1576577} & \formatNumber[round-precision=4]{0.1606972} & \formatNumber[round-precision=4]{0.2554745} & \formatNumber[round-precision=4]{0.3969849} \\
    & \hiergat & \formatNumber[round-precision=4]{0.0664464} & \formatNumber[round-precision=4]{0.1159887} & \formatNumber[round-precision=4]{0.1220429} & \formatNumber[round-precision=4]{0.9491185} & \formatNumber[round-precision=4]{0.0913095} & \formatNumber[round-precision=4]{0.0562211} & \formatNumber[round-precision=4]{0.0923423} & \formatNumber[round-precision=4]{0.0903248} & \formatNumber[round-precision=4]{0.6858407} & \formatNumber[round-precision=4]{0.0793973} & \formatNumber[round-precision=4]{0.4099099} & \formatNumber[round-precision=4]{0.4275391} & \formatNumber[round-precision=4]{0.6615776} & \formatNumber[round-precision=4]{1.0000000} \\
    & \dmatcher & \formatNumber[round-precision=4]{0.0591351} & \formatNumber[round-precision=4]{0.1042905} & \formatNumber[round-precision=4]{0.1118978} & \formatNumber[round-precision=4]{0.8463718} & \formatNumber[round-precision=4]{0.0567983} & \formatNumber[round-precision=4]{0.0854613} & \formatNumber[round-precision=4]{0.0292793} & \formatNumber[round-precision=4]{0.0627462} & \formatNumber[round-precision=4]{0.6470588} & \formatNumber[round-precision=4]{0.0779954} & \formatNumber[round-precision=4]{0.4256757} & \formatNumber[round-precision=4]{0.4481681} & \formatNumber[round-precision=4]{0.5922078} & \formatNumber[round-precision=4]{0.4623116} \\
    & \hmatcher & \formatNumber[round-precision=4]{0.0503411} & \formatNumber[round-precision=4]{0.0802748} & \formatNumber[round-precision=4]{0.0834608} & \formatNumber[round-precision=4]{0.9392546} & \formatNumber[round-precision=4]{0.0086569} & \formatNumber[round-precision=4]{0.0506273} & \formatNumber[round-precision=4]{0.0405405} & \formatNumber[round-precision=4]{0.0293457} & \formatNumber[round-precision=4]{0.6734694} & \formatNumber[round-precision=4]{0.0574369} & \formatNumber[round-precision=4]{0.2612613} & \formatNumber[round-precision=4]{0.2740272} & \formatNumber[round-precision=4]{0.5511364} & \formatNumber[round-precision=4]{1.0000000} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \walamz~}}
    & \ditto & \formatNumber[round-precision=4]{0.0250543} & \formatNumber[round-precision=4]{0.0971858} & \formatNumber[round-precision=4]{0.0976012} & \formatNumber[round-precision=4]{0.9379355} & \formatNumber[round-precision=4]{0.0390661} & \formatNumber[round-precision=4]{0.0311995} & \formatNumber[round-precision=4]{0.1383616} & \formatNumber[round-precision=4]{0.1304388} & \formatNumber[round-precision=4]{0.7810026} & \formatNumber[round-precision=4]{0.0353393} & \formatNumber[round-precision=4]{0.1578422} & \formatNumber[round-precision=4]{0.1557477} & \formatNumber[round-precision=4]{0.7790698} & \formatNumber[round-precision=4]{1.0000000} \\
    & \hiergat & \formatNumber[round-precision=4]{0.0258767} & \formatNumber[round-precision=4]{0.1463761} & \formatNumber[round-precision=4]{0.1345393} & \formatNumber[round-precision=4]{0.9600204} & \formatNumber[round-precision=4]{0.0306233} & \formatNumber[round-precision=4]{0.0259996} & \formatNumber[round-precision=4]{0.1688312} & \formatNumber[round-precision=4]{0.1556869} & \formatNumber[round-precision=4]{0.7816092} & \formatNumber[round-precision=4]{0.0288772} & \formatNumber[round-precision=4]{0.1303696} & \formatNumber[round-precision=4]{0.1240960} & \formatNumber[round-precision=4]{0.7771084} & \formatNumber[round-precision=4]{0.0000000} \\
    & \dmatcher & \formatNumber[round-precision=4]{0.0377159} & \formatNumber[round-precision=4]{0.1610030} & \formatNumber[round-precision=4]{0.1673286} & \formatNumber[round-precision=4]{0.8332366} & \formatNumber[round-precision=4]{0.0599565} & \formatNumber[round-precision=4]{0.0140516} & \formatNumber[round-precision=4]{0.1028971} & \formatNumber[round-precision=4]{0.0545092} & \formatNumber[round-precision=4]{0.6908078} & \formatNumber[round-precision=4]{0.0482802} & \formatNumber[round-precision=4]{0.3676324} & \formatNumber[round-precision=4]{0.3730055} & \formatNumber[round-precision=4]{0.6710526} & \formatNumber[round-precision=4]{1.0000000} \\
    & \hmatcher & \formatNumber[round-precision=4]{0.0214808} & \formatNumber[round-precision=4]{0.1198746} & \formatNumber[round-precision=4]{0.1207576} & \formatNumber[round-precision=4]{0.9406378} & \formatNumber[round-precision=4]{0.0520903} & \formatNumber[round-precision=4]{0.0229369} & \formatNumber[round-precision=4]{0.1288711} & \formatNumber[round-precision=4]{0.1294780} & \formatNumber[round-precision=4]{0.7896104} & \formatNumber[round-precision=4]{0.0317548} & \formatNumber[round-precision=4]{0.0369630} & \formatNumber[round-precision=4]{0.0435302} & \formatNumber[round-precision=4]{0.7088608} & \formatNumber[round-precision=4]{0.0000000} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPGogS~}}
    & \ditto & \formatNumber[round-precision=4]{0.0417208} & \formatNumber[round-precision=4]{0.0218842} & \formatNumber[round-precision=4]{0.0261769} & \formatNumber[round-precision=4]{0.9943404} & \formatNumber[round-precision=4]{0.0043948} & \formatNumber[round-precision=4]{0.0445106} & \formatNumber[round-precision=4]{0.0079545} & \formatNumber[round-precision=4]{0.0022551} & \formatNumber[round-precision=4]{0.9330872} & \formatNumber[round-precision=4]{0.0510580} & \formatNumber[round-precision=4]{0.0661616} & \formatNumber[round-precision=4]{0.0560378} & \formatNumber[round-precision=4]{0.9228585} & \formatNumber[round-precision=4]{0.0050251} \\
    & \hiergat & \formatNumber[round-precision=4]{0.0382689} & \formatNumber[round-precision=4]{0.0160378} & \formatNumber[round-precision=4]{0.0153315} & \formatNumber[round-precision=4]{0.9968356} & \formatNumber[round-precision=4]{0.0025589} & \formatNumber[round-precision=4]{0.0438299} & \formatNumber[round-precision=4]{0.0212121} & \formatNumber[round-precision=4]{0.0092096} & \formatNumber[round-precision=4]{0.9349169} & \formatNumber[round-precision=4]{0.0488706} & \formatNumber[round-precision=4]{0.0219697} & \formatNumber[round-precision=4]{0.0233680} & \formatNumber[round-precision=4]{0.8791322} & \formatNumber[round-precision=4]{0.6231156} \\
    & \dmatcher & \formatNumber[round-precision=4]{0.0470777} & \formatNumber[round-precision=4]{0.0831641} & \formatNumber[round-precision=4]{0.0696028} & \formatNumber[round-precision=4]{0.9859389} & \formatNumber[round-precision=4]{0.0432199} & \formatNumber[round-precision=4]{0.0527080} & \formatNumber[round-precision=4]{0.0940657} & \formatNumber[round-precision=4]{0.0786143} & \formatNumber[round-precision=4]{0.9490892} & \formatNumber[round-precision=4]{0.0707030} & \formatNumber[round-precision=4]{0.1391414} & \formatNumber[round-precision=4]{0.1399734} & \formatNumber[round-precision=4]{0.9352031} & \formatNumber[round-precision=4]{1.0000000} \\
    & \hmatcher & \formatNumber[round-precision=4]{0.0447968} & \formatNumber[round-precision=4]{0.0356740} & \formatNumber[round-precision=4]{0.0351347} & \formatNumber[round-precision=4]{0.9959054} & \formatNumber[round-precision=4]{0.0065181} & \formatNumber[round-precision=4]{0.0565425} & \formatNumber[round-precision=4]{0.0561869} & \formatNumber[round-precision=4]{0.0514161} & \formatNumber[round-precision=4]{0.9259758} & \formatNumber[round-precision=4]{0.0526075} & \formatNumber[round-precision=4]{0.0494949} & \formatNumber[round-precision=4]{0.0476417} & \formatNumber[round-precision=4]{0.9031936} & \formatNumber[round-precision=4]{0.1959799} \\
    \midrule

    \multirow{4}{*}{\rotatebox[origin=c]{90}{ \small \DBLPACM~}}
    & \ditto & \formatNumber[round-precision=4]{0.0106186} & \formatNumber[round-precision=4]{0.0054744} & \formatNumber[round-precision=4]{0.0051546} & \formatNumber[round-precision=4]{0.9987834} & \formatNumber[round-precision=4]{0.0008359} & \formatNumber[round-precision=4]{0.0103183} & \formatNumber[round-precision=4]{0.0060866} & \formatNumber[round-precision=4]{0.0038916} & \formatNumber[round-precision=4]{0.9688889} & \formatNumber[round-precision=4]{0.0125531} & \formatNumber[round-precision=4]{0.0117131} & \formatNumber[round-precision=4]{0.0129752} & \formatNumber[round-precision=4]{0.9707207} & \formatNumber[round-precision=4]{0.0050251} \\
    & \hiergat & \formatNumber[round-precision=4]{0.0084030} & \formatNumber[round-precision=4]{0.0085360} & \formatNumber[round-precision=4]{0.0063838} & \formatNumber[round-precision=4]{0.9999134} & \formatNumber[round-precision=4]{0.0002981} & \formatNumber[round-precision=4]{0.0046326} & \formatNumber[round-precision=4]{0.0048126} & \formatNumber[round-precision=4]{0.0023191} & \formatNumber[round-precision=4]{0.9843400} & \formatNumber[round-precision=4]{0.0113218} & \formatNumber[round-precision=4]{0.0226123} & \formatNumber[round-precision=4]{0.0199241} & \formatNumber[round-precision=4]{0.9886364} & \formatNumber[round-precision=4]{0.8442211} \\
    & \dmatcher & \formatNumber[round-precision=4]{0.0063796} & \formatNumber[round-precision=4]{0.0051026} & \formatNumber[round-precision=4]{0.0054396} & \formatNumber[round-precision=4]{0.9993873} & \formatNumber[round-precision=4]{0.0018270} & \formatNumber[round-precision=4]{0.0068598} & \formatNumber[round-precision=4]{0.0048126} & \formatNumber[round-precision=4]{0.0003691} & \formatNumber[round-precision=4]{0.9854423} & \formatNumber[round-precision=4]{0.0043971} & \formatNumber[round-precision=4]{0.0067235} & \formatNumber[round-precision=4]{0.0114964} & \formatNumber[round-precision=4]{0.9806157} & \formatNumber[round-precision=4]{0.0000000} \\
    & \hmatcher & \formatNumber[round-precision=4]{0.0081192} & \formatNumber[round-precision=4]{0.0105233} & \formatNumber[round-precision=4]{0.0119347} & \formatNumber[round-precision=4]{0.9995538} & \formatNumber[round-precision=4]{0.0005278} & \formatNumber[round-precision=4]{0.0093301} & \formatNumber[round-precision=4]{0.0054496} & \formatNumber[round-precision=4]{0.0047909} & \formatNumber[round-precision=4]{0.9844098} & \formatNumber[round-precision=4]{0.0110709} & \formatNumber[round-precision=4]{0.0226123} & \formatNumber[round-precision=4]{0.0196499} & \formatNumber[round-precision=4]{0.9830508} & \formatNumber[round-precision=4]{0.0000000} \\
    






    
    \bottomrule
    \end{tabular}
    %}
    \caption{Mninization of EOD\\ \mhm{{\\ This table is after calibration with respect to minimizoing EOD, we can't include the other (respct to EO, PR)} \\3 digit precision was not enough} \mostafa{The tables look fantastic, great job! But I suggest adding the increase or decrease as you see in DP. The table will grow in length which is fine, we can break the table into three or frou tables and e.g., show Distribional parity in one, and AUC and delta auc in another and tau=0.5 in another. But each will have increase/decrease added. These tables can take only a column, not the entire textwidth. I can help with breaking the tables if you agree and can update the numbers.Also the results for the last three datasets is not good! Is it because lambda is optimized for all measures? Do we get better results if we do that per measure? Almost in all, there is no significant improvement. Only AMZ-GOG is good.}}
        \vspace{-3mm}
        \label{tab:bias-after1}
    \end{table*}






\amzgog
\walamz



==> problem_definition.tex <==
\section{Problem Definition}\label{sec:problem}
%https://reader.elsevier.com/reader/sd/pii/S0195669817300860?token=4FC3D18950004077BB7E95179333CFD2C1750D2BD3F6C0110F8CD62F2F64CEC7D4E6C23B3F2E5212F2D3A4EF7BF04910&originRegion=us-east-1&originCreation=20230214022052

%The concept of data repair commonly pertains to modifying a database to adhere to a predefined set of constraints. As discussed in Section~\ref{sec:intro}, in some applications involving a data distribution, the distribution is expected to conform to certain CI constraints; it becomes pertinent to 'repair' the distribution itself, irrespective of its representation, to meet the requirements of these CIs. In this section, we formalize our intended meaning behind the notion of distribution repair.


Given a database $\db$ that is inconsistent with a CI constraint $\sigma: (\mb X \indep \mb Y \mid \mb Z)$, our objective is to resolve this inconsistency by updating the attribute values of each datapoint in $\db$ to derive a repaired database $\hat{\db}$ which is consistent with $\sigma$. To ensure minimal distortion and maintain the utility of the data, we assume we are given a user-defined cost function that quantifies the cost of updating a datapoint (this cost function generalizes the minimality criteria in update-based data repair in databases~\cite{bertossi2006consistent}). Leveraging the principles of OT, our goal is to develop a data cleaner, envisioned as a transport map, that repairs $ \db $ at a minimum cost. Next, we define the problem of learning an optimal data cleaner for a CI constraint.

\begin{definition}[CI Data Cleaner] \label{df:repair} \em
Consider a database $ \db = \{ \mb v_i \}_{i=1}^n $ that violates a CI constraint $ \sigma $, i.e., $ \db \not \models \sigma $, and a user-defined cost function $ c: \mathcal{V} \times \mathcal{V} \rightarrow \mathbb{R}_{\geq 0} $ that assigns a cost to transforming or perturbing one tuple in 
$\mathcal{V}$ to another tuple in 
$\mathcal{V}$. The \textit{CI data cleaner} of $ \db $ with respect to $ \sigma $ is a transport map $ T^* : \mathcal{V} \rightarrow \mathcal{V} $ that transforms $ \db $ into a database $ \hat{\db} = T^*(\db) = \{ \hat{\mb v_i} = T^*(\mb v_i) \}_{i=1}^n $ such that $ \hat{\db} \models \sigma $ and has the minimum transportation cost, i.e., $ T^* $ is the solution to the following constrained optimization problem: {\small\begin{align}
    \arg\min_{T} \sum_{i=1}^{n} c(\mb v_i, T(\mb v_i)) & 
    & \text{s.t.} \quad T(\db) \models \sigma. \label{eq:detrepair}
\end{align}
}
\end{definition}

We illustrate an optimal data cleaner with an example: 

\begin{example} \label{ex:odcexexis}\em     Let's consider a database $\db_1 = \{(0, 0, 1)$, $(1, 0, 1)$, $(0, 1, 1)$, $(0, 1, 0)\}$ defined over binary variables $X$, $Y$, and $Z$. $\db_1$ violates the CI constraint $\sigma:Y \indep Z$ because the probability $P_{Y,Z}(1, 0)$ is $\frac{1}{4}$, which is not equivalent to the product of the marginal probabilities $P_{Y}(1) = \frac{2}{4}$ and $P_Z(0) = \frac{1}{4}$. Further, suppose cost is measured using Euclidean distance.  
    An optimal CI repair can be obtained using the transport map $T$, which maps $(0, 0, 1) \rightarrow (0, 0, 0)$ and other tuples to their current values. As a result, by updating one attribute value, $T$ transforms $\db_1$ into a repaired database 
    $\hat{\db_1} = \{(0, 0, 0), (1, 0, 1), (1, 1, 0), (0, 1, 1)\}$,
    which is consistent with $\sigma$. %\mostafa{Do we mention L1 norm cost? Thanks, commented this} \babak{added Euclidean distanc}
\end{example}


% Mostafa: I corrected an error in the example that was due to assuming Z, X, Y as the order in the distribution, as opposed to X,Y,Z
 

However, the CI data cleaner defined in Definition~\eqref{df:repair} might not lead to a minimum cost repair. This is especially true if $\db$ is a bag, which is typically the case with databases used for ML. These databases are either bags or projections onto a subset of features that yield a bag. We illustrate this with an example:

\begin{example}\label{ex:odcexnotexis}
\em Continuing with Example~\ref{ex:odcexexis}, now consider a database $\db_2 = \{(1, 0, 0), (1, 0, 1), (1, 1, 0), (1, 1, 0)\}$, which is now a bag, and is inconsistent with the constraint $Y \indep Z$. Similarly, $\hat{\db_2} = \{(1, 0, 0)$, $(1, 0, 1)$, $(1, 1, 0)$, $(1, 1, 1)\}$ is a minimum cost repair for $\db_2$, obtained by modifying only one attribute value. However, no transport map exists that can transport $\db_2$ into $\hat{\db_2}$ simply because $(1, 1, 0)$ cannot be mapped to both itself and $(1, 1, 1)$. Upon close examination, it becomes evident that no transport map can lead to a repair for $\db_2$ with cost 1. 
\end{example}

%Moreover, for an instance $\db_3 = \{(1, 0, 0), (1, 1, 1)\}$, it is evident that a repair consistent with Definition~\ref{df:repair} does not exist. 

% Mostafa: The same error was in the above example.

\paragraph{\bf Probabilistic Optimal Data Cleaner} As demonstrated in Example~\ref{ex:odcexnotexis}, the transport map defined in Definition~\ref{df:repair} does not always yield the minimum cost repair (although it can always produce a trivial repair by mapping every tuple to a single tuple, which completely distorts the distribution). Indeed, it's possible for the minimum cost repair to be outside the feasible region defined by the problem in Equation~\eqref{eq:detrepair}. Drawing from the Kantorovich relaxation of OT, we shift our approach to seeking a transport plan, or transport coupling, denoted as $\pi(\mb v', \mb v)$, as an alternative to a deterministic transport map $T$. Here, the marginal distribution $\pi(\mb v) = \pr^{\db}$ represents the empirical distribution of the database $\db$, and $\pi(\mb v')$ is the target distribution that is consistent with the CI constraint. This transport plan yields a probabilistic mapping, $\pi(\mb v' \mid \mb v)$, which probabilistically updates a data point $\mb v \in \db$ to $\mb v'$ following the mapping. The repaired database is then obtained by applying this mapping to $\db$, by sampling. In essence, Definition~\ref{df:repair} transitions into a problem where the aim is to (1) identify a transport plan $\pi(\mb v', \mb v)$ that pushforwards the distribution $\pi(\mb v) = \pr^{\db}$, i.e., the empirical distribution associated with $\db$ into one consistent with the CI constraints, and (2) among all distributions with the same support and consistent with the constraint, find the distribution $\pi(\mb v')$ with the minimum OT distance to $\pi(\mb v) = \pr^{\db}$. Formally, an {\em optimal probabilistic data cleaner} for CI constraint seeks to clean data using a probabilistic mapping $\pi( \mathbf{v}' \mid \mathbf{v})$ associated with a transport plan or probabilistic coupling $\pi( \mathbf{v}', \mathbf{v})$, obtained by solving the following optimization problem:  
%

\vspace{-0.3cm}
{\small
\begin{align}\hspace{-3mm}
    \arg\min_{\pi} \sum_{i=1}^{d_{\Dom V}} \sum_{j=1}^{d_{\Dom V}} c(\mathbf{v}_i, \mathbf{v}'_j) \pi(\mathbf{v}_i, \mathbf{v}'_j)
    & \ \ \text{s.t.} \ \ \pi(\mathbf{v}) = \pr^{\mathrm{\db}}, \; \pi(\mb v') \models \sigma. \label{def:potr}
\end{align}}
%
\noindent The feasible region of the optimization problem defined in Equation~\ref{def:potr} consists of all possible probability distributions that satisfy the constraint, hence including a distribution associated with a minimal cost repair. Therefore, one can find a mapping that transforms the empirical distribution of $\db$ into a consistent distribution with the minimum cost. Moreover, the optimal probabilistic mapping, derived from solving Equation~\ref{def:potr}, provides an approach for probabilistic data cleaning. For large datasets, samples drawn from this probabilistic cleaner will lead to a dataset \( \hat{\db} \) whose empirical distribution \( \pr^{\hat{\db}} \) closely aligns with the target distribution \( \pr(\mathbf{v'}) \), in line with the law of large numbers. Consequently, the resulting dataset is approximately consistent with the constraint. In ML applications, this level of approximation is generally adequate.






\begin{figure}
\begin{tikzpicture}[node distance=1.5cm, auto, thick, scale=0.7, every node/.style={scale=0.7}]

\tikzstyle{vertex}=[circle, fill=white, draw, minimum size=1cm, drop shadow={shadow xshift=0.05cm, shadow yshift=-0.05cm, opacity=0.5}]

\node[vertex] (a) {$(1, 0, 0)$};
\node[vertex] (b) [below=0.2cm of a] {$(1, 0, 1)$};
\node[vertex] (dots1) [below=0.2cm of b, scale=0.8] {$\vdots$};
\node[vertex] (c) [below=0.2cm of dots1] {$(1, 1, 0)$};

\node[vertex] (a') [right=1.5cm of a] {$(1, 0, 0)$};
\node[vertex] (b') [below=0.2cm of a'] {$(1, 0, 1)$};
\node[vertex] (dots2) [below=0.2cm of b', scale=0.8] {$\vdots$};
\node[vertex] (c') [below=0.2cm of dots2] {$(1, 1, 0)$};
\node[vertex] (d') [below=0.2cm of c'] {$(1, 1, 1)$};


% Draw the 1 probabilities
\draw[-,red] (a) -- (a') node[midway,above,scale=1.5,yshift=-1pt] {1/4};

\draw[->,blue, dashed, bend left=40] (a) to node[midway,above,scale=1.5,yshift=0pt] {1} (a');

\draw[-,red] (b) -- (b') node[midway,above,scale=1.5,yshift=0pt] {1/4};

\draw[->,dashed, blue, bend left=-40] (b) to node[midway,above,scale=1.5,yshift=0pt] {1} (b');

\draw[-,red] (c) -- (c') node[midway,above,scale=1.5,yshift=0pt] {1/4};

\draw[->, dashed,blue, bend left=40] (c) to node[midway,above,scale=1.5,yshift=0pt] {1/2} (c');

\draw[-,red] (c) -- (d') node[midway,below,scale=1.5,yshift=0pt] {1/4};
\draw[->, dashed, blue, bend left=-40] (c) to node[midway,below,scale=1.5,yshift=0pt] {1/2} (d');

% Draw the 0 probabilities with labels
\foreach \source in {dots1, a, b, c} {
    \foreach \dest in {dots2, a', b', c', d'} {
        \ifx\source\dest\else% do not label the arrows we already labeled
            \draw[-, dotted, gray, opacity=0.5] (\source) -- (\dest);
        \fi
    }
}

% Connect the dots with gray lines to all other nodes

% Adding labels and braces
\node[scale=2, above=0.2cm of a] (v) {$\mathbf{v}$};
\node[scale=2, above=0.2cm of a'] (v'){$\mathbf{v'}$};

 \node[left=-4.5cm of a, anchor=west] (lhstable) {
\begin{tabular}{@{}ccS[table-format=1.2]@{}}
\toprule
\Large{$\mathbf{v}$} & \Large{$\pi(\mathbf{v})$} \\
\hline
\midrule
$(1, 0, 0)$ & 1/4 \\
$(1, 0, 1)$ & 1/4 \\
\rowcolor{blue!10}
$(1, 1, 0)$ & 1/2 \\
\bottomrule
\end{tabular}
};

% Bottom Table
\node[below=0.5cm of lhstable, anchor=north] (rhstable) {
\begin{tabular}{cc}
\toprule
\Large $\mathbf{v}'$ &  \Large $\pi(\mathbf{v}')$ \\
\hline
\midrule
$(1, 0, 0)$ & 1/4 \\
$(1, 0, 1)$ & 1/4 \\
\rowcolor{blue!10}
$(1, 1, 0)$ & 1/4 \\
\rowcolor{blue!10}
$(1, 1, 1)$ & 1/4 \\
\bottomrule
\end{tabular}
}; 
\end{tikzpicture}
\caption{Graphical representation of the plan $\pi(\mb v, \mb v')$ for $\db_2$. Nodes represent elements in $\mc V$. Labeled red edges indicate joint probabilities $\pi(\mb v, \mb v')$, while dashed directed edges depict the probabilistic mapping $\pi(\mb v \mid \mb v')$. Only nodes and edges with non-zero probabilities are shown for clarity.}
\label{fig:tpexample}
\end{figure}


%\draw[decorate, decoration={brace, amplitude=2pt, raise=-5pt}, yshift=-5pt] 
%  (-1.2,-3.3,-12) -- (0.2,-3.3,-12) node [midway, above, yshift=-15pt] {};

% LHS Table for marginal distribution



\begin{example}\label{ex:odcexnotexis2} \em
Consider $\db_2 = \{(1, 0, 0)$, $(1, 0, 1)$, $(1, 1, 0)$, $(1, 1, 0)\}$ from Example~\ref{ex:odcexnotexis}. The probabilistic mapping $\pi(\mb v, \mb v')$ is graphically represented in Figure~\ref{fig:tpexample}, which depicts the bipartite graph constructed from the elements of the domain $\mc V$. Labeled red edges illustrate the joint probabilities $\pi(\mb v, \mb v')$, while dashed directed edges showcase the corresponding probabilistic mapping $\pi(\mb v \mid \mb v')$. The graph only includes nodes and edges for which $\pi(\mb v, \mb v')$ and $\pi(\mb v \mid \mb v')$ are non-zero to maintain clarity. It's evident that the marginal distribution $\pi(\mb v)$ displayed in Figure~\ref{fig:tpexample} matches the empirical distribution $\pr^{\db_2}$ associated to $\db_2$. Furthermore, $\pi(\mb v \mid \mb v')$ primarily maps all elements to themselves with a probability of 1. However, it transports half of the mass from $(1,1,0)$ to itself and the other half to $(1,1,1)$ to repair the constraint violation. This results in a distribution $\pi(\mb v')$ consistent with the constraint. Notably, the OT cost of this repair is $1/4$ since just $1/4$ of the mass with cost 1 transitions from $(1,1,0)$ to $(1,1,1)$. 

The mapping $\pi(\mb v \mid \mb v')$ can be employed to clean $\db_2$ probabilistically. Due to the limited sample size, this doesn't guarantee consistency. Still, for a larger database, the repaired database becomes representative of $\pi(\mb v')$ and hence becomes consistent with the constraint. To illustrate this, consider another database $\db_3$ echoing the tuples in $\db_2$, but each tuple is now replicated $n$ times. This mirrors the empirical distribution of $\db_2$ and still violates the constraint. In such a scenario, repairing $\db_3$ with $\pi(\mb v \mid \mb v')$ likely results in a consistent database. Probabilistically repairing the $2n$ instances of $(1, 1, 0)$ in $\db_3$ through the mapping $\pi(\mb v'\mid \mb v)$ can be interpreted as a sequence of $2n$ Bernoulli trials with a 1/2 probability. On average, this yields $n$ tuples of $(1, 1, 0)$ and $n$ tuples of $(1, 1, 1)$, ensuring consistency with the constraints.
\end{example}

% \babak{can you fix the spacing here}

\vspace{-3mm}
\paragraph{\bf Discussion on Complexity} Designing scalable algorithms to solve the optimization problem outlined in \eqref{def:potr} and subsequently computing optimal repairs for CI constraints presents significant challenges. A straightforward approach entails exploring the vast space of all distributions consistent with the CI, computing OT distance in relation to the empirical distribution of $\db$, and identifying the optimal solution. This method, however, is not feasible primarily due to the intractable nature of the space of consistent distributions. Furthermore, as discussed  in~\ref{sec:intro}, the computation of OT is computationally demanding. In our context, the transport plan involves \(d_{\Dom V}^2\) variables, thereby exacerbating the inherent complexity. 


Although a detailed complexity analysis of the optimization problem~\ref{def:potr} is not addressed in this paper, it is worth noting that our problem is akin to the computation of minimum update-based repair (U-repair) for MVDs~\cite{bertossi2006consistent}. U-repair aims to identify a repair that necessitates the fewest attribute value modifications to enforce an MVD. Specifically, given a database \(D\) with attributes \(XYZ\) and an MVD \(X \twoheadrightarrow Y\), the decision problem is whether \(D\) has an optimal U-repair with no more than \(k\) modifications. This decision problem can be translated to our repair challenge by presuming a uniform distribution over \(D\), considering a cost function \(c(x, y, z, x', y', z')\) that enumerates the number of modifications required to obtain $(x', y', z')$ from $(x, y, z)$, and checking if \(D\) can achieve an optimal repair at a cost lesser than \(k\) given the conditional independence \(X \indep Y \mid Z\). Under the specified assumptions, it is easy to check \(D \models (X \indep Y \mid Z) \) if and only if \(D \models X \twoheadrightarrow Y\).  While there's extensive literature on the U-repair problem for Functional Dependencies~\cite{kolahi2009approximating,livshits2020computing}, to the best of our knowledge, it hasn't been studied for MVDs. %Furthermore, our repair problem, as described in~\cite{salimi2019interventional}, is also related to the rank-one matrix approximation problem, which is known to be NP-hard.







%\begin{example}\label{ex:odcexnotexis2}
%Consider the database $\db_2 = \{(1, 0, 0), (1, 0, 1), $ $  (1, 1, 0), (1, 1, 0)\}$, as highlighted in Example~\ref{ex:odcexnotexis}. The probabilistic coupling $\pi(\mb v, \mb v')$ is graphically represented in Figure~\ref{fig:tpexample}. In this figure, nodes correspond to elements $v$ and $v'$ from the domain $\mc V$, while labled red edges illustrate the joint probabilities $\pi(\mb v, \mb v')$ and  the dashted directed edges represent $\pi(\mb v \mid \mb v')$. Theb graph only present nodes and edges for which $\pi(\mb v, \mb v')$ and $\pi(\mb v mid \mb v')$are non-zero for clarify. One can validate that the marginal distribution $\pi(\mb v)$ shown in~\ref{fig:tpexample} corrponds to the emperical distribution $\pr^{\db_2}$ asscoiated with $\db_2$. Furthere, the probabalitic mppimg $\pi(\mb v \mid \mb v')$ mappis all element to themself with probabality 1 but transport halph of the mass for $(1,1,0)$ to itself $(1,1,0)$ and halph of it to $(1,1,1)$ to fix the vioilation of the constraint and creates a distribution $\pi(\mb v')$ which is consistent with constraints. Further the OT cost of this repair is only $1/4$ since only 1/4 of the mass with cost 1 moved from $(1,1,0)$ to $(1,1,1)$. The mapping $\pi(\mb v \mid \mb v')$ could be used to probabalisticaly clean $\pi(\mb v \mid \mb v')$. Cosider a database $\db_3$ with the same tuples as $\db_2$ but suppose now each tuple has multiplicity $n$ which define the same emeprical distribution as $\db_2$ and violate the constraint. In this case cleaning $\db_3$ with $\pi(\mb v \mid \mb v')$ yeilds a consistent database with high probabality, since cleaning 2.n $(1, 1, 0)$ occurances of $\db_3$ using the mapping $\pi(\mb v'\mid \mb v)$ cna be seen as a 2.n bernouli trial with probabality 1/2 which in expetation generates $n$ tuples $(1, 1, 0)$ and $n$ yuples $(1, 1, 1)$
%\end{example}





%This approach allows for a more flexible representation, where each point in the original database $\db$ can potentially be associated with multiple points in the repaired database $\hat{\db}$ with varying probabilities. By considering these probabilistic associations, we aim to achieve a repair that, on average, maintains consistency with the given constraints, while also minimizing the overall distortion or cost. This probabilistic framework offers a robust alternative, especially in cases where deterministic mappings fail to provide a viable solution.





%\babak{Update till here}
%The set of possible repairs, $\repair(\pr,\sigma)$ in Definition~\ref{df:repair}, is always non-empty. This is because some probability distributions always satisfy $\sigma$, and a coupling can be found between them and $\pr$. Additionally, the set of possible repairs can contain more than one repair because of possibly more than one way of transporting the same mass amount from $\pr$ to different positions in $\prQ$ to satisfy $\sigma$, resulting in different $\prQ$. When considering an optimal repair $\prQ$, there may be more than one possible coupling $\coupleM$ in $\coupling(\pr,\prQ)$ since masses from different positions of $\pr$ can be transported to generate the same optimal repair $\prQ$. 


%\subsection{The Connection with Data Repair Problem}

%The problem in Definition~\ref{df:repair} specifies an optimal repair as a probability distribution. However, the term ``repair'' is often used in data cleaning and consistent query answering to refer to a repaired database obtained from minimally changing an input database to comply with some constraints, e.g., database integrity constraints. In our problem, we can also assume we start with a database $D$ and define the repair problem for finding a repaired database. $D$ is often assumed i.i.d. samples from an unknown target distribution $P^*$. The input distribution $P$ in our problem can be considered the estimation of $P^*$ using $D$ obtained through any estimation technique, e.g., the empirical distribution of $D$. Therefore, $P$ may depart from $P^*$ due to sampling biases, noise, or other forms of errors. Knowing that $P^*$ complies with a particular CI constraint, the repair problem can be seen as a problem of repairing $P$ to a distribution $Q$ that is closer to $P^*$ and does not suffer from biases and errors resulting from the sampled records in $D$. Therefore, one might use the repaired distribution $Q$ as a close distribution to $P^*$ or sample from it to generate a repair database $D'$ for any downstream task, as we do in our experiments. One can consider the coupling that gives $Q$ as a probabilistic map that given $D$ maps it to a probabilistic database where each record has a probability attached to it.

%in $D$ or  from this distribution is available. Therefore, we must define a repaired database $D_\prQ$ for an input database $D_\pr$ w.r.t. a set of IC constraints $\Sigma$. To do this, we assume that given $D_\pr$, we can estimate a probability distribution $\hat{\pr}$ and obtain its repair $\hat{\prQ}$ as defined in Definition~\ref{df:repair}. $\hat{\prQ}$ can be used in different ways to define $D_\prQ$. The following definition formalizes the concept of a repaired database w.r.t. a CI constraint.

%An optimal repair of $\prQ$ can be obtained by solving the following optimization problem that seeks for a push forward $\push$ of $\pr$  such that $Q =\push_{\#}(P)$
%
%\begin{equation} \min_{Q =\push_{\#}(P)} \quad \ot(Q,P) \ \ \ \text{s.t.} \ \ \ X \indep Y \mid_{Q} Z \label{eq:distrep}\end{equation}
% Now we define the problem of optimal repair for a database:

%\begin{definition}[Database Repair] \label{df:dbrepair}
%Consider an input database $D_\pr$ that is sampled from an unknown distribution with probability distribution $\pr$, and let $\hat{\pr}$ be an estimation of $\pr$ obtained from $D_\pr$.\footnote{We use the empirical distribution $\hat{\pr}$ to estimate the underlying distribution $\pr$, but our approach can be adapted for other estimations.} Given a CI constraint $\sigma: X \indep Y \mid Z$ that is inconsistent with $\hat{\pr}$, let $\repair(\hat{\pr},\sigma)$ be the set of optimal repairs of $\hat{\pr}$ w.r.t. $\sigma$ as defined in Definition~\ref{df:repair}.

%A {\em repaired database} for $D_\pr$ w.r.t. $\sigma$ is a tuple-independent probabilistic (TIP) database $D_q$ that is obtained from an optimal repair $\hat{q} \in \repair(\hat{\pr},\sigma)$. We use $\repair(D_\pr,\sigma)$ to refer to the set of repaired databases.

%For every tuple $t\in D_p$ and for every repair $D_q \in \repair(D_\pr,\sigma)$ obtained from a coupling $\coupleM \in \coupling(\hat{p},\hat{q},\sigma)$, we define its repair as a TIP database $D^{t,\coupleM}q$ that consists of a subset of tuples in $D_q$, where the probabilities of the tuples are obtained from the coupling $\coupleM$ for the optimal repair $\hat{q}$.\boxtheorem
%\end{definition}

%In Definition~\ref{df:dbrepair}, a TIP database refers to a probabilistic database in which each tuple has a constant probability independent of the probabilities of the other tuples in the database~\cite{suciu2011probabilistic}. If a database repair $D_q$ is obtained from a transport map, as in the Monge formulation, the probability of every tuple $t$ in $D_q$ is $1$, making $D_q$ a typical database obtained from applying the map on tuples in $D_p$. In this case, each tuple $t\in D_q$ has equal probability $1$. Definitions~\ref{df:repair} and \ref{df:dbrepair} can be extended to a set of CI constraints $\Sigma$ instead of a single constraint $\sigma$.

%e introduced the notations $\hat{\pr}$ and $\hat{\prQ}$ to define the concept of repaired database $D_q$. In the rest of the paper, we will use the simpler notations $\pr$ and $\prQ$ to refer to the original distribution and its repaired version, respectively.

%We define the following types of {\em data repairs} for $D$ w.r.t. $\sigma$: 
%\begin{itemize}
%    \item The {\em exact data repair} $D_\mathcal{T}$ is obtained from a pushforward that generates $\hat{\prQ}$ if $\hat{\prQ}=\pushRepair(\hat{\pr},\sigma)$:
%\begin{align*}
%D_\mathcal{T}=\{t'\mid\exists t\in D\wedge \mathcal{T}(t)=t'\}    
%\end{align*}
%\noindent where $\mathcal{T}$ is the pushforward.
%\item The {\em most-likely repair} is obtained from the coupling $\coupleM$ from the optimal repair $\hat{\prQ}$ as follows:
%\item The {\em probabilistic repair} is ...
%\end{itemize}

%is to transform $D_{P}$ into another database $D_{Q}$ that can be seen as a sample from a repaired distribution $Q$ of $\pr$.

%Hence, one can obtain an optimal repair for an inconsistent $D$ using the transformation obtained by solving the optimization problem in Equation~\ref{eq:distrep}.


%Let $\Delta(\Datap \times \Datap)$ be the set of all possible distributions over the product space $\Dom \Datap = \Dom X \times \Dom Y \times \Dom Z \times \Dom W$. Let $P \in \Delta(\Datap)$ be a distribution that is inconsistent with the CI constraint $X \indep Y \mid Z$. We define an {\em optimal repair} of $\pr$ w.r.t. $X \indep Y \mid Z$ as a distribution $Q \in \Delta(\Datap)$ such that among all $Q' \in \Delta(\Datap)$ that are consistent with $X \indep Y \mid Z$, $\ot(Q,P) \leq \ot(Q',P)$. An optimal repair of $\pr$ can be obtained by solving the following optimization problem that seeks for a pushforward such that $Q = \mathcal{T}_{\#}(P)$ is an optimal repair:

%\begin{equation}
%\min_{Q =\push_{\#}(P)} \quad \ot(Q,P) 
%\ \ \ \text{s.t.} \ \ \  X \indep Y \mid_{Q} Z 
%\label{eq:distrep}
%\end{equation}


%We say a database $D$ drawn from a distribution $\pr$ is {\em inconsistent} with a CI constraint $X \indep Y \mid Z$ if, $\pr$ is inconsistent with it, i.e,  $X \not \indep Y \mid_{P} Z$.  The problem of finding an {\em optimal repair} of $D$ wrt. the constraint $X \indep Y \mid Z$ is to transform $D$ into another database $D'$ that can be seen as sample from $Q$ an optimal repair of P. Hence, one can ibtain an optimal repair for an incosistent $D$ using the transofrmation obtained by solving the optimization problem in Equation~\ref{eq:distrep}. 



\ignore{


%\vspace{-3mm}
%\begin{align} 
%     \Tilde{T} = \argmin_{T\in \push}\dist (P,\Tilde{P})
%  \hspace{1cm} \text{such that\ } \Tilde{P} \models \Sigma   \label{eq:repairproblem}
%\end{align}

%A repaired database $\Tilde{D}$ is  drawn from $\popul$ to a {\em repaired database} $\drepair=\{\rdatap_i=\trans(\datap_i)\}_{i=1}^n$ that corresponds to a {\em repaired data distribution} $\modifpopul$, such that the distribution $\pr_{\rdatap \sim \modifpopul }(\rdatap)$ is {\em minimally different} from 

%Specifically, the problem of computing optimal repairs to a database $\dtrain$ wrt a set of CI constraints $\Sigma$ is how to transform the database $\dtrain$ to another database $\drepair$ via an optimal data cleaner $\optrans$ obtained by solving the following optimization problem: 
%
%\setlength{\abovedisplayskip}{0pt}{\small\setlist{nosep}\vspace{-.1cm} \begin{align}      \optrans = \argmin_{\trans}\dist\!\left(\pr_{\rdatap \sim \modifpopul }(\rdatap), \pr_{\datap \sim \popul }(\datap) \right)&&& \text{s.t.\ } \pr_{\rdatap \sim \modifpopul }(\rdatap) \models \Sigma   \label{eq:repairproblem}\end{align} }
%

\noindent In Equation~\ref{eq:repairproblem}, $\push$ is the set of possible pushforwards from the discrete space $\bDom V$ to itself, and $\dist$ is a function that measures the distance between two distributions, e.g., the family of {\em f-divergence} that generalizes the relative entropy (aka the Kullback-Leibler (KL) divergence)~\cite{csiszar1967information}, and  {\em optimal transport} measures % measures WHAT? 
such as the {\em Wasserstein distance}~\cite{villani2009optimal}. 

A repair $\Tilde{D}$ for $D$ w.r.t. $\Sigma$ is a database obtained from applying the pushforward $\Tilde{T}$ on $D$:

\vspace{-3mm}
\begin{align}\label{eq:repair}
\Tilde{D}=\{\Tilde{v}_j|\exists v_i \in D \wedge \Tilde{v}_j=\Tilde{T}(v_i)\}    
\end{align}

\noindent The idea of the repair in Equation~\ref{eq:repair} is as follows. Assuming the pushforward $\Tilde{T}$ converts the distribution $\pr$ to $\Tilde{P}$ that satisfies $\Sigma$, the repair $\Tilde{D}$, which is obtained from mapping data in $D$ using $\Tilde{T}$ will also respect the CI constraints.  

%We define a repair of $D$ as the database obtained from applying the pushforward $\Tilde{T}$ on $D$:

%Given $D$, we assume a known probability distribution $P_D$ as an estimation of $\Delta$ obtained from $D$. 

The {\em degree of inconsistency} of a distribution $\pr$ from a constraint $(\mb X \indep \mb Y \mid \mb Z)$ can be quantified by measuring the distance between $\pr_{X,Y,Z}(\mb x,  \mb y, \mb z )$ and  $\pr_{Y,Z}(\mb y, \mb z )\pr_{X\mid Z}(\mb x, \mb z )$, which is zero iff $(\mb X \indep \mb Y \mid_{\pr} \mb Z)$; for KL divergence, it is in correspondence with conditional mutual information~\cite{yeung1997framework}.




\babak{We should check whether the problem of finding optimal cardinality repair for saturated MVDs is in correspondent to our repair for a particular cost function.}
}

==> related_work.tex <==
\section{Related Work}

Our research connects with two main areas of study.
\vspace{-2mm}
\paragraph{\bf Data Cleaning for Conditional Independence}
Data cleaning in the database domain traditionally revolves around enforcing integrity constraints, such as functional dependencies and conditional functional dependencies~\cite{livshits2020computing, kolahi2009approximating, bohannon2006conditional, DBLP:conf/icdt/LivshitsK21}. Nonetheless, the domain of data cleaning for conditional independence has only recently gained attention. Notable works in this emerging field include~\cite{salimi2019interventional} and \cite{yan2020scoded}. SCODED~\cite{yan2020scoded} employs statistical constraints to detect errors within datasets but primarily focuses on ranking individual data tuples based on their relevance to conditional independence violations, differing from our data-centric approach. On the other hand, \cite{salimi2019interventional} aims to find optimal repairs for conditional independence violations, involving the addition or removal of tuples to satisfy the constraint. However, their method lacks the application of specific statistical divergence or distance measures to assess the quality of the repaired data. In a somewhat distinct vein,~\cite{ahuja2021conditionally} utilizes generative adversarial networks (GANs) to generate data adhering to conditional independence constraints. Their primary objective is to train these generative models effectively, particularly emphasizing the minimization of Jensen–Shannon divergence in continuous data. However, their focus is on training generative models rather than cleaning existing data.
\vspace{-2mm}
\paragraph{\bf Fairness and Optimal Transport}
Algorithmic fairness research has primarily focused on detecting and mitigating biases in machine learning models, utilizing pre-, post-, and in-processing techniques. Pre-processing methods~\cite{Caton2020FairnessIM}, aim to eliminate bias from training data before model training. While model-agnostic approaches such as~\cite{NIPS2017_6988, feldman2015certifying, salimi2019interventional} exist, they often lack insights into the root causes of biases. These strategies typically address basic fairness criteria and may not delve into enforcing conditional independence tests or incorporating optimal transport methods. Notably,~\cite{gordaliza2019obtaining} employs the Wasserstein barycenter for pre-processing training data to achieve statistical parity but doesn't specifically address the complexities of conditional statistical inference in high-dimensional datasets, distinguishing it from our approach. \cite{silvia2020general} employs optimal transport as a regularizer during ML model training, focusing on a different aspect than our data cleaning objective. Additionally, studies like~\cite{si2021testing, black2020fliptest} use optimal transport to quantify unfairness, making them less aligned with our core research goal.




==> revision.tex <==
\section*{Revision Letter}

\vspace{1cm}
\noindent {\bf Dear Reviewers,}

We are grateful for your insightful feedback, which has significantly contributed to enhancing the quality of our paper. We first address the meta-reviewer's overall feedback and then offer comprehensive responses to each reviewer's comments individually. Changes implemented in the manuscript based on specific feedback are marked in the revised version using the following color scheme:


\begin{itemize}
\item \metareviewer{Meta reviewer and changes mentioned by multiple reviewers in Plum}\vspace{-1.5mm}
\item \reviewerone{Reviewer 1 in Orange}\vspace{-1.5mm}
\item \reviewertwo{Reviewer 2 in Cyan}\vspace{-1.5mm}
\item \reviewerthree{Reviewer 3 in Blue} 
\end{itemize}


\subsection*{Response to Meta Reviewer}

\begin{itemize}
    \item {\bf Required Changes:} The reviewers have provided detailed feedback on their concerns. They have all indicated the important changes that are required in a revision as part of Q14 in their review. Kindly address all points raised therein. Please pay particular attention to clarify the novelty of optimal transport repairs for conditional independence constraints in light of Dasu et al. Kindly use the reviewers responses to author feedback Q17 for additional context/clarification.
    \metareviewerA{Thank you for your advice on how to respond to the reviewers' feedback. We have thoroughly examined their suggestions and worked to address them within the given timeframe. About the study by Dasu et al.~\cite{dasu2012statistical}, we've included a new section, Section~\ref{sec:distortion}, in our paper, where we briefly discuss their method for evaluating cleaning strategies through statistical distortion. We also conducted experiments to test our system, \sys, and compared it with other baselines using this approach.}
    
    \item {\bf Optional Changes:} The reviewers have pointed out several minor issues in addition to the required changes. We hope the authors will be able to address these issues as well.
    \metareviewerA{We have addressed all the comments from the reviewers, including their minor remarks.}
\end{itemize}


\subsection*{Response to Reviewer \#1}

\reviewerone{Thank you for your constructive comments. Please find our responses to your comments below.}

\begin{itemize}
        \item {\bf 12. Availability:} The cleaning methods/experimental data are not included in the repository.
        \revieweroneA{We have made our code and data available for both fairness and data-cleaning applications in the same repository used for the initial submission.}
        
        
        \item {\bf 13. Minor remarks:} Page 2: “This challenge becomes especially pronounced when considering „ Why pronounced?, Generally the introduction appears verbose. Page 6: lesser. Page 9: a ML model. Page 9: before data cleaning, “as demonstrated in [45]” dot is missing. Table 3 -> time unit is missing, based on the figure 8a it should be seconds.
        \revieweroneA{We have addressed all these remarks. The introduction has been revised for conciseness, removing unnecessary words and making our arguments more direct.}
        
    \item {\bf 14. List required changes for a revision:} Open the balck box for data cleaning experiments, include more sophisticated baselines for imputation. Dasu et al., deeper analysis with prior work see O4. 
    \revieweroneA{Thank you for suggesting these helpful improvements. To make our cleaning experiments clearer, we have added a new paragraph (the third paragraph in Section~\ref{sec:exp-cleaning}) explaining how we introduced attribute noise and missing values. To include more sophisticated methods, we have incorporated GAIN, which uses Generative Adversarial Networks~\cite{yoon2018gain}, and Hyperimputation, a method that integrates multiple imputation techniques, blending traditional iterative imputation with deep learning~\cite{jarrett2022hyperimpute}. We chose GAIN since it is a popular state-of-the-art method for imputation and Hyperimpute due to its generality that integrates and outperforms multiple imputation methods. For cleaning attribute noise, we added Baran~\cite{mahdavi2020baran} as an advanced data cleaning method that utilizes comprehensive context information, including the value, co-occurring values, and attribute type, to generate correction candidates with high precision. These new methods are all leading representative methods in their respective areas of data cleaning and imputation. The explanation of the baselines has been revised in the paragraph before Section~\ref{sec:tuning}. The updated experimental results are detailed in the two paragraphs immediately before Section~\ref{sec:distortion}.}
    
    \reviewerone{The work in Dasu et al.~\cite{dasu2012statistical} does not introduce a new cleaning method but rather provides a framework for comparing them. We have introduced a new section, Section~\ref{sec:distortion}, where we discuss the framework and conduct experiments to evaluate \sys and compare it with our baselines using this framework.}

%\babak{Dasu et al. dfoes not introduce a daat cleaning techniqe. They introduce a framwork for vealuting cleaning tehcniqes ... }
    
    \item{\bf 17. Response to author feedback:} Regarding ``R1O3: Please inform us if there are specific baselines you recommend for comparison.'' On a second thought, I think it is sufficient to compare to the cleaning algorithm suggested in the statistical distortion paper: Dasu et al.
    \revieweroneA{As noted earlier, Dasu et al. do not introduce a new cleaning method and offer a framework for comparing cleaning strategies~\cite{dasu2012statistical}. Please refer to our earlier response and Section~\ref{sec:distortion} for detail.}

    \item {\bf 8. Describing in detail all opportunities for improvement:}
    \begin{itemize}
        \item {\bf O1:} Text: The reader needs backgrounds in statistics, optimization problems, linear algebra (matrix scaling), and fairness, right in the introduction. Although the story is clear, sometimes a higher-level description could be helpful to understand the details. For example, the part about the Sinkorn algorithm needs more context. Particularly, algorithm 1, lines 4, and 5 need more description. Also, an example describing the algorithm would be helpful. (line 6). - Kantorovich formulation: this coupling/joint distribution is confusing. - Example 3.4 could have been more descriptive. The probabilities and number of attributes are not easily understandable at the first glance.
        \revieweroneA{To enhance understanding, we have provided extra details about Kantorovich formulation, regularized Optimal Transport (OT), and the Sinkhorn algorithm in Section~\ref{sec:ot}. For clearer explanation, we've also added Example~\ref{ex:reg-ot} and Figure~\ref{fig:sinkhorn} to illustrate the main ideas of regularized OT.}
        
        \item {\bf O2:} Experiments: The dataset generation, particularly generating training sets is a black box. The authors mentioned that they deliberately injected noise that led to violations of constraints, but they did not mention the way they generated the noise. Also, the injection of missing values not at random (MNAR) is not clear. Probably an example could be helpful.
        \revieweroneA{To create a dependency between two attributes through attribute noise, we introduce random noise into one based on the values of the other. For adding missing data, our approach depends on the type. In MAR scenarios, where an attribute's missingness is influenced by another attribute, we decide to add missing values based on the other attribute's values in the same record. In MNAR cases, where an attribute's missingness is affected by its own value and other attributes, we randomly select records and determine missingness based on these factors. This method systematically creates relationships between attributes, effectively incorporating noise and addressing different missing data situations. This is added in the third paragraph in Section~\ref{sec:exp-cleaning}.}
  %\babak{MOSTAFA WILL WORK ON THIS}      
        
        \item {\bf O3:} Reporting the metrics such as F-Score of cleaning could be also useful.
        \revieweroneA{We have included F1-score results, shown in Figures~\ref{fig:car-f1-noise} and \ref{fig:boston-f1-noise}, along with AUC. The F1-score data shows that \sys still performs better than the baseline methods. However, F1-score results are more variable compared to AUC, mainly because of the constant 0.5 threshold in F1-score calculations. Generally, AUC is a more consistent measure for evaluating accuracy across various thresholds.}
        %\babak{MAKE IT SHORTER} 

        %\babak{AS EXPLAINED ABOVE .... IN TERMS OF DISTURTION ONE OF THEY PROPOSED MAINLY W DISTANCE WHICH CONICENDES WITH ARE DIONG ... IN ADITION THEY PROPOSED  AMETHOD FOR EVALUATION ... WE DID EXACTLY THE SAME SHIT}
        \item {\bf O4:} The paper lacks contextualization with regard to previous work by Dasu et al. Why cant we use their metric for statistical distortion?
        \revieweroneA{Please refer to our earlier response and the new section, Section~\ref{sec:distortion}.}

        \item {\bf O5:} The distinction between fairness and cleaning experiments is a bit unclear. Are you only pertubating dirty cells in the latter?
  \revieweroneA{\sys functions similarly in both data cleaning and fairness applications, with a few distinctions. In data cleaning, we explore two settings: 1) incorporating background knowledge about erroneous attributes into the cost function of \sys, and 2) allowing the algorithm to autonomously determine which attributes to clean without assumptions. While \sys effectively reduces spurious correlations in both settings, it demonstrates notably superior performance when operating without assumptions about erroneous attributes, as depicted in Figure~\ref{fig:noise} and detailed in a new paragraph in Section~\ref{sec:exp-cleaning}. In the fairness application, we refrain from making assumptions about erroneous attributes, but we do not perturb sensitive attributes to facilitate the computation of fairness metrics.}
        %\babak{OUR ALGORUTHMS DOES NOT ASSUME ANY BACKGROUND KNBOLEDGE ON DIRTY CELLS IT MERELY ACCES THE CONSTRAINTS AS INPUT AND PURTUBE THE ENTIURE DATA WRT THE COST FUNCTION, HOWEVER, ANY BACKGROUND KNOLEDGE REGARDING THE ERROHNNOUD DATTRIBUTE COULD BE INCIRPORATED TO THE COST FUCNTON SUCH THAT THE OTCLEAN ONLY FOCUS ON REPARING PARTICULAR SUBSETCS OF ATTRIBUTES ....  IN OUR EXPERIMENST WE DID NOT DISTINGUISH BETWEEN THE FAIRNESS ANCD  CLENAING AOPLICTAIIN AND MNERELY PURTURB DATA  ... IN FAIRNESS I GUESS WE HAVE SOEM RESTRICTIONS ... SECOND THOUGHT: IT SEEMS THAT FOR CLEANING WE HAVE BNOTH SETTING REFER TO THE RELEVENT PLOTS. }
    \end{itemize}
\end{itemize}

\subsection*{Response to Reviewer \#2}
\begin{itemize}
%\item {\bf 13. Minor Remarks:} Page 2: nageable -> manageable
%\reviewertwoA{Thank you for pointing out the typo. We have now corrected it.}
\item {\bf 8. Details of opportunities for improvement}
\begin{itemize}
    \item {\bf O1:} In the medical diagnosis and job application examples in the introduction, I think it would be good to clarify the distinction between correlation and causation. My understanding is that clearly there is correlation, say between ZIP code and recovery, but the point is to make sure no causal relationship can be picked up by a model. So when doing data cleaning, we need to pick data repairs that don't accidentally introduce causal relationships. I think these issues are implicitly mentioned throughout the paper, but it might help to mention them more explicitly.
    \item {\bf O2:} Also, perhaps an example would help to show the difference between a causal relationship and a correlation in a small dataset (maybe similar to example 3.2 that appears later, but preferably using more realistic data). When I was reading the introduction, statements like "given a dataset that violates a CI constrain" weren't immediately obvious to me. Intuitively, how do we tell that a dataset violates a CI constraint as opposed to just a correlation constraint?
\reviewertwoA{Thank you for your feedback. We did not intend to imply that data cleaning methods introduce causal relationships, as causal relationships are inherent facts about the domain, not a result of data manipulation. The example aimed to demonstrate how data quality issues might introduce spurious correlations. These correlations, although not causal, can be mistakenly picked up by ML models, which do not distinguish them from genuine causal relationships. We have revised the example to clarify this distinction and appreciate your suggestion to enhance the paper's accessibility. This revision aims to more accurately convey how data quality and cleaning can impact the inferential processes of ML models. Thank you for your valuable input.}
    
\end{itemize}
\end{itemize}

\subsection*{Response to Reviewer \#3:}

\begin{itemize}
%\item {\bf 12. Availability:} The provided content reflects the authors' diligent efforts in addressing the issue of violations of conditional independence in data cleaning. The theoretical innovation of formulating the repair problem as a regularized optimization problem, along with the development of an algorithm that guarantees convergence, is particularly noteworthy. In addition, the empirical results that show the method's ability to maintain fairness while ensuring high predictive performance are impressive. However, there are opportunities to enhance the comprehensiveness of the research: 
%\begin{enumerate}
%    \item The use of semi-synthetic datasets for evaluation is a good start, but including a broader range of diverse and real-world datasets could provide a more comprehensive demonstration of the method's applicability and robustness.
%    \item While the iterative algorithm inspired by Sinkhorn's matrix scaling algorithm is innovative, providing more detailed performance metrics on larger datasets would help us better understand its scalability limitations and practical utility.
%\end{enumerate} 
%\reviewerthreeA{}

\item {\bf Minor remarks:}
\begin{enumerate}
   % \item Reference Formatting: Some references appear to be inconsistently formatted. For example, Reference [15] differ in style from others. Consistency in reference formatting is recommended.
%    \reviewerthreeA{Alireza}
    \item Caption Details: The captions for some figures, such as Figure 4 and Figure 3, could be more descriptive to provide better context for the reader.For Figure 3, adding a brief description of the key elements shown in the figure and their relevance to the data cleaning process would be helpful. For Figure 4, a more detailed caption explaining the significance of the results depicted and how they support the paper's conclusions would enhance reader comprehension. These changes would provide clearer context and make the figures more informative.
\reviewerthreeA{Thank you for the suggestion. We updated the captions for Figures~\ref{fig:fairness} and \ref{fig:fairness-measures} to include more detail. Note that Figures~\ref{fig:fairness} and \ref{fig:fairness-measures} are Figures~3, and 4 in your comment, with numbers, increased due to a new figure.}
    
\item Clarification of Algorithm Steps
The description of Algorithm 1 in the manuscript is somewhat brief, which might be challenging for readers unfamiliar with the topic. A more detailed explanation, including the purpose of each step, how they interconnect, and their role in the overall data cleaning process, would be beneficial. For instance, elaborating on how the algorithm handles different types of data irregularities and the rationale behind each computational step would make this section more informative and accessible to a broader audience.
\reviewerthreeA{We added more explanation to help understand the Sinkhorn algorithm. Please see our response to R1.O1.}

\end{enumerate}
\item {\bf 14. List of required changes:} Based on the identified opportunities for improvement (O1, O2, O3), here are the required changes for a revision:
%\babak{EXPLAIN WHJY WE USE SYTHETIC DATA AND ITS LIMITATION....}
\begin{enumerate}
    \item Refinement in Dataset Selection and Processing (O1): Section 6.3: Enhance the discussion on the use of semi-synthetic datasets. Acknowledge and address the limitations in capturing the complexity and diversity of real-world data scenarios. Provide a more in-depth analysis of the biases potentially introduced by using the most frequent values (MF) and KNN for imputation, especially in complex missing data patterns. Discuss in detail the specific performance losses that may occur due to the deliberate introduction of non-random noise and the injection of MAR and MNAR types of missing data.
    \reviewerthreeA{We appreciate your point about semi-synthetic data and we added discussion about our choice of semi-synthetic datasets and its limitations to the second paragraph in Section~\ref{sec:exp-cleaning}.}
    
    \item Improvement in Model Generalization and Assessment (O2): Section 6.3: Revise the approach for assessing model generalization. Consider incorporating noise and missing values in the test set to more accurately reflect real-world conditions and avoid overly optimistic evaluations. Conduct a thorough examination and quantification of the model's performance deterioration in the presence of noisy and incomplete data.
    \reviewerthreeA{As noted earlier, we have added a brief discussion about semi-synthetic datasets, focusing on their limitations and impact. To show how our results can be broadly applied, we have also integrated three sophisticated imputation and cleaning methods. For more details, please refer to our response in R1.14.}
    
    \item Enhancing Scalability and Addressing Dataset Diversity (O3): Provide a detailed explanation of the performance and feasibility of the proposed iterative algorithm for calculating optimal transport distances on very large datasets. Validate the method across a more diverse range of real-world datasets to offer a comprehensive assessment of its practicality. Outline future work aimed at expanding the applicability of the proposed methods to larger and more varied datasets, thereby demonstrating scalability and robustness.
    \reviewerthreeA{The runtime and scalability of our algorithm are primarily determined by the number of attributes in the CI constraints, not the size of the data. The transport plan's size remains constant regardless of data size and varies only with the number of involved attributes. A crucial aspect of our experiments is the domain size, which depends on both the number of attributes in the CI constraints and their possible value range. Our experiments demonstrate that the runtime is largely unaffected by data size, a finding we've omitted in our report due to its straightforward nature. We have discussed this in the highlighted paragraph in Section~\ref{sec:sys-exp}.}
\end{enumerate}
\end{itemize}

%\babak{HIGHLIGHT TH EXPERIMENT IN THE EXPERIMENT RELEVENT TO NUMBER OF ATTRIBUTE. SAY WE ALSO RAN THE EXPEIRMENT BY INCERAISNG THE SIZE OF DATA FROM .. TO .... HOWEVER, AD DICUSSES .... THIS OUWLD NOT AFFETC THE DIMENTIONALITY OF INPUTS OF THE ALGORIUTHM HENCE THE RUNNING IS CONTAST WE DID NOT INCLUDE THE PLOYT BECAUSE ... }

==> unsaturated.tex <==
\vspace{-0.1cm}\paragraph{\bf Unsaturated CI Constraints}\label{sec:unsat} So far, we assumed that \(\sigma: X\indep Y \mid Z\) represents a saturated CI constraint, implying \(\st{V}=\{X,Y,Z\}\). However, in many real-world scenarios, especially with high dimensional data, CI constraints may not be saturated.

For unsaturated constraints, we split \(\st{V}\), the set of attributes in the database \(D\), into two sets: \(\st{U}=\{X,Y,Z\}\) (the attributes in \(\sigma\)) and \(\st{W}=\st{V}\setminus \st{U}\) (those not in \(\sigma\)). A naive method is to compute a transport plan \(\coupleM\) of size \(d^2_{\Dom V}\), considering all attributes in \(\st{V}\), including \(\st{W}\). Adapting methods from Section~\ref{sec:methods} for this scenario is straightforward but computationally expensive with high-dimensional data.

A more efficient strategy is to run \mainAlg for the marginal distribution \(P^D_\st{U}\) instead of \(P^D\). This results in a smaller transport plan \(\coupleM_s\) of size \(d^2_{\Dom U}\) compared to \(\coupleM\). With \(\coupleM_s\), we construct \(\coupleM\) as follows: \(\coupleM(\vt{v},\vt{v}')=0\) if \(\vt{w}\neq \vt{w}'\), and \(\coupleM(\vt{v},\vt{v}')=\coupleM_s(\vt{u},\vt{u}') P_{\st{W} \mid \st{U}}(\vt{w}\mid \vt{u})\) otherwise. This ensures no additional transport cost for moving masses between different values of \(\st{W}\) as there is no mass moved for \(\vt{w}\neq \vt{w}'\). Thus, the cost associated with \(\coupleM\) is the same as \(\coupleM_s\), making it optimal if \(\coupleM_s\) is optimal. Note that this requires the cost function to satisfy some basic properties, such as the cost of \(\vt{u}\vt{w} \rightarrow \vt{u}'\vt{w}\) being equal to the cost of \(\vt{u} \rightarrow \vt{u}'\), which is satisfied by the Euclidean distance and other cost functions in our work. Additionally, the use of \(P_{\st{W} \mid \st{U}}(\vt{w}\mid \vt{u})\) ensures that \(\coupleM\) satisfies the marginal constraint \(P^D(\vt{v})=\coupleM(\vt{v})\). The resulting distribution \(Q\) from \(\coupleM\) satisfies \(\sigma\) as its marginal is \(Q_{\st{U}}\) which is known to satisfy \(\sigma\).

 



%We propose that the optimal solution can be expressed as \(Q_{\st{V}}(\vt{v}) = Q_{\st{U}}(\vt{u}) \times Q_{\st{W}\mid \st{U}}(\vt{w}|\vt{u})\), where \(Q_{\st{W}\mid \st{U}}\) is formulated as:%\begin{equation} Q_{\st{W}\mid \st{U}}(\vt{w}\mid \vt{u}') = \sum_{\vt{u} \in \dom{U}} \coupleM(\vt{u},\vt{u}') \times P_{\st{W} \mid \st{U}}(\vt{w}\mid \vt{u}) \label{eq:saturation} \end{equation}

%In the above equation, \(\coupleM\) denotes the reduced-size transport plan. The outcome of \eqref{eq:saturation} provides an optimal plan for \(P^D\), incorporating all variables \(\st{V}\). This is because the transport cost of $\coupleM$ and obtaining $Q_{\st{U}}$ will be the same as the transport cost of the larger transport plan for generating $Q_\st{V}$. This is because the conditional probability $P_{\st{W} \mid \st{U}}$ is used to convert the marginal $Q_{\st{U}}$ to $Q_{\st{V}}$, which means no additional cost is incurred for adding $\st{W}$ to the transport plan. \ignore{For example, if the incurred cost of moving mass from $\vt{u}=(0,0)$ to $\vt{u}'=(0,1)$ is $\coupleM(\vt{u},\vt{u}')=a$,  the same cost will be incurred for moving mass from $\vt{v}_1=(0,0,0)$ and $\vt{v}_2=(0,0,1)$ to $\vt{v}'_1=(0,1,0)$ and $\vt{v}_2=(0,1,1)$. }We have labeled this efficient method as the Saturation approach and will demonstrate its superior runtime performance compared to the ``Naive'' method in the experiments in Section~\ref{sec:sys-exp-opt}.

